Results from a Practical Deployment of the MyZone Decentralized P2P Social Network

This paper presents MyZone, a private online social network for relatively small, closely-knit communities. MyZone has three important distinguishing features. First, users keep the ownership of their data and have complete control over maintaining their privacy. Second, MyZone is free from any possibility of content censorship and is highly resilient to any single point of disconnection. Finally, MyZone minimizes deployment cost by minimizing its computation, storage and network bandwidth requirements. It incorporates both a P2P architecture and a centralized architecture in its design ensuring high availability, security and privacy. A prototype of MyZone was deployed over a period of 40 days with a membership of more than one hundred users. The paper provides a detailed evaluation of the results obtained from this deployment.

==> designChallenges.tex <==
\section{Design Goals and Challenges}
\label{ch:designGoalsAndChallenges}

In this section we describe the main goals that are guiding the design of MyZone, and describe the challenges facing it.
 
\subsection{Design Goals}
\label{sec:goals}

In the introduction, we described the following shortcomings for the existing OSNs:

\begin{enumerate}
\item User privacy violations on behalf of the OSN service providers.
\item Government imposed censorship aimed at repressing popular uprisings by means of preventing the OSN services being used as tools for facilitating these movements.  
\item User confusion and frustration resulting from abundance of different OSNs, and frequently changing policies and features that are imposed by the OSN service providers.
\item The undeniable threat of hijacking user information from centralized data centers by targeted attacks.  
\end{enumerate} 

The eminent need for a next generation of OSNs that addresses these shortcomings has motivated MyZone towards the following goals:

\begin{itemize}

\item It should preserve user privacy by ensuring that users own their own data, and no central authority or third party can access user information without explicit permission from the user.  

\item User privacy preservation should not come at the cost of losing functionalities provided by existing OSNs. Therefore, it should support all primary functionalities of a conventional OSN like Facebook. These include the ability to establish and revoke friendships, sharing contents and comments with friends at different levels, and participating in discussions.


\item It should be highly resilient in face of malicious attacks as well as infrastructure failures caused by unpredictable causes. The OSN continues to function in isolated islands (which will be referred to as {\it ``local deployment''}) while facing network partitioning, and possesses self healing properties, by automatically reconciling the states after the partition has been restored.

\item It should tolerate a high rate of churn due to mobile users, and seek to provide
near 24/7 availability of user profiles (best effort).


\item Due to the growing trend of switching to smartphones and tablet computers, the underlying computing platform consists of traditional desktops and laptops with high bandwidth network connections, as well as portable devices with restricted resources. To deal with the latter, the system should be designed to be minimally demanding of the limited resources of portable devices, and should incorporate power/resource management techniques.

\end{itemize}


\subsection{Challenges}
\label{sec:challenges}

The shortcomings of existing OSNs, demand a distributed architecture for the next generation of OSNs. Based on the distributed architecture, the assumptions mentioned earlier, and the design goals, we identify six key challenges in the design, implementation, and deployment of
MyZone: availability, resiliency, routing, connectivity, security, and traffic optimization and power management.


\subsubsection{Availability Challenges}
\label{subsec:availability}


An important property of OSNs is that a user profile is always available regardless of whether that user is currently online or not. This is made possible by storing user profiles in a central server/data center that is available all the time. Providing this property in a distributed OSN, where user profiles are not replicated at any central server is further complicated by high rate of churn. Overcoming this challenge is perhaps the key to the success of a distributed OSN. 

In the absence of a central server, profile replication must be considered as an intrinsic part of the system design. The key question is where should a user profile be replicated, i.e. how to select {\bf mirrors} for replicating a user profile. There are two design choices with this regard:
mirroring a user profile on a set of devices belonging to random users; or replicating the user profile on a set of devices belonging to users that are trusted by the owner of the profile.

Deploying DHTs would use the first approach to replicate user profiles. Although DHTs have proven to be a success, dealing with availability issues, they are mostly used to replicate contents that are not going to be modified. Even in some cases where the replicated content is modified, the modifying entities are not restricted to a specific selection of users. One possibility of implementing this restriction is by sharing a common key between all friends of a user and replicate the encrypted profiles, using this common key. 

There are three problems with this approach. First, even assuming that the shared keys are not going to be obtained by non-friend users, revoking a friendship translates into revoking the shared key, issuing a new key, sending it to all friends, and finally re-encrypting the entire profile using the new key. This process is very inefficient considering the fact that revoking friendships can occur frequently. 

Second, a simple modification of the user profile by a friend e.g. a one word comment, may translate into sending the entire encrypted profile to the friend and re-encrypting it by the friend after making the modification, and sending it back to the mirror. This process is also inefficient and would result in unnecessary use of bandwidth, traffic, and power resources. 

Even if the updates are encrypted in a way that prevents this to happen e.g. sending encrypted updates to the mirror and appending them to the end of the encrypted profile, it is still very hard to send a particular part of the profile from the mirror to the friend since the entire profile is encrypted and the mirror does not know which chunks of the encrypted profile should be sent.

Finally and probably most importantly it would be impossible to implement application level permissions e.g. who can see what part of the user profile or modify it, since the profile is encrypted using a {\it shared} key. Furthermore, the mirror will not be able to impose those permissions since it does not know the key. Of course sharing the key with an unknown mirror would compromise user privacy and profile integrity. Thus, because of the special features and functionalities of OSNs, DHTs can not and should not be used to host OSN services.

The only feasible solution would be the second approach and we believe that candidate designs must investigate the second approach, where users find other trustworthy users amongst existing friends to replicate their profiles. Finding friends who are willing to be mirrors and convincing them  to serve as mirror either through social ties, or proposing incentives, would be an interesting problem on its own.


In addition to the issue of selecting mirrors, there are several other aspects of replication management that must be addressed given the dynamic nature of the system due to churn. These  are: 
\begin{enumerate}
\item When and how profile updates are propagated to other mirrors.
\item How to maintain replica consistency among all mirrors.
\item What type of replica consistency is appropriate for this application.
\item Whether a user profile is completely or partially replicated at different mirrors.
\item Whether the mirrors themselves should be prioritized as primary, secondary,  and so on. 
\end{enumerate}

\subsubsection{Resiliency Challenges}
\label{subsec:resiliency}

The proposed system is intended to be deployed in an infrastructure that is vulnerable due to: {\bf 1)} mobile users with widely varying Internet connections,  and {\bf 2)} malicious entities that may try to partition the social network or bring down the system. Hence the system needs to be resilient in such environments and must be self-healing.


\subsubsection{Routing Challenges}
\label{subsec:routing}

A key requirement of the OSN is that, users must be able to locate their (mobile) friends and establish connections when they join the system. This is further complicated by the high rate of churn.

One approach is that all users register their IP addresses on a rendezvous server when they join the system . A user then, would contact this server
with appropriate credentials to determine the current IP addresses of her friends. This solution suffers from the major drawback of the server being a single point of failure.  In addition, that single rendezvous server needs to be trusted since it would have a global view of the social graph and it can derive social relationships, which is not desirable. 

A second approach is to use a distributed hash table (DHT) scheme to hash an individual's username to a particular rendezvous server for lookup, but then we have to implement an efficient mechanism that would prevent the rendezvous server in charge of a user $i$ from disclosing user $i$'s IP address to users that are not her friends. This is to prevent targeted attacks on $i$. Our design would focus on the second approach.

\subsubsection{Connectivity Challenges}
\label{subsec:connectivity}

The user devices participating in the OSN are mostly behind firewalls or NATs (around 90\%). NATs are divided into four types: 
\begin{itemize}
\item Full Cone NAT: Once an internal address (iAddr:iPort) is mapped to an external address (eAddr:ePort), any packets from iAddr:iPort will be sent through eAddr:ePort and any external host can send packets to iAddr:iPort by sending packets to eAddr:ePort.
\item Address Restricted Cone NAT: Once an internal address (iAddr:iPort) is mapped to an external address (eAddr:ePort), any packets from iAddr:iPort will be sent through eAddr:ePort and an external host (hAddr:any) can send packets to iAddr:iPort by sending packets to eAddr:ePort only if iAddr:iPort has previously sent a packet to hAddr:any. "Any" means the port number doesn't matter.
\item Port Restricted Cone NAT: Once an internal address (iAddr:iPort) is mapped to an external address (eAddr:ePort), any packets from iAddr:iPort will be sent through eAddr:ePort and an external host (hAddr:hPort) can send packets to iAddr:iPort by sending packets to eAddr:ePort only if iAddr:iPort has previously sent a packet to hAddr:hPort.
\item Symmetric Cone NAT: The NAT mapping refers specifically to the connection between the local host address and port number and the destination address and port number and a binding of the local address and port to a public side address and port. Any attempts to change any one of these fields requires a different NAT binding. 

This is the most restrictive form of NAT behavior under UDP, and it has been observed that this form of NAT behavior is becoming quite rare, because it prevents the operation of all forms of applications that undertake referral and handover.
\end{itemize} 

Configuring firewalls and NATs to forward requests to a particular internal host is not common knowledge for many users, and may not be possible in some cases. An alternative way to avoid reconfiguring NAT is called NAT traversal. 

A common method of NAT traversal is for an internal host to send a UDP packet to an outside host first, and depending on the type of NAT, the internal host may be able to receive connections from all, or a subset of external hosts afterwards. This method is commonly known as UDP hole punching. Except for the full cone NAT, the use of UDP hole punching limits the extent of external hosts that can connect to the internal host. In fact UDP hole punching is impossible on symmetric cone NATs. 

Although full cone NATs are commonly used by home users, a good portion of users are behind other kinds of NATs. Connecting peers that are behind NATs is another challenge that must be addressed, otherwise the application of such OSN would be limited to very few users that have access to public IP addresses.


\subsubsection{Security Challenges}
\label{subsec:security}

Our design needs to provide the following security guarantees:

\begin{itemize}
\item {\it Confidentiality}: Prevent the disclosure of profile information to any user that is not a friend.
\item {\it Integrity}: A user profile can only be viewed and modified by her friends.
\item {\it Availability}: The OSN is resilient against DDoS attacks and URL/IP filtering, and user profiles are {\it ``almost always''} available.
\item {\it Authenticity}: Every modification of a user profile is authenticated.
\item {\it Consistency}: A weakly consistent view of the profile is always available.
\end{itemize}

The consistency and availability guarantees are bound to be best effort as the benefits gained through absolute availability and total consistency are not worth the added complexity in the design of the OSN.  This tradeoff is described in the CAP Theorem\cite{brewer2000towards}, which stipulates that there is a tradeoff in distributed systems between consistency, availability, and partitioning (in our case due to attacks and/or user churn).


\subsubsection{Traffic Optimization and Power Management Challenges}
\label{subsec:traffic_power}

As mentioned in section \ref{ch:assumptions}, users may use a wide range of devices to participate on the OSN, including smartphones and other portable devices, laptops and desktop computers. In addition each user device may also act as a mirror for another user. A key challenge is to provide availability while dealing with resource-constrained devices.  Portable devices are primarily constrained by energy and bandwidth limitations, though memory and CPU limitations also play a factor.  A challenge is to develop a replication strategy that takes into account these limitations while providing availability and resiliency. One strategy is to leverage more resource-rich devices, i.e. online desktops, to support the bulk of mirroring duties, and to use mobile mirroring only as a strategy of last resort.

Heterogeneity of device resources and their limitations call for optimized resource usage of the system, especially with regards to traffic and power management schemes. Such a system should try to save as much energy and bandwidth as possible (memory and CPU are not as critical as power and bandwidth in portable devices). For example, a pushing scheme would prove less efficient in terms of power and traffic optimization as opposed to a pulling scheme when it comes to reflecting user profile updates to friends.

==> implementation.tex <==
\section{Implementation}
\label{ch:implementation}

We described the design of MyZone in Chapters \ref{ch:systemDesign} and \ref{ch:securityMeasures}. In this chapter we provide more details on the implementation of MyZone by describing the code components, interfaces and classes that implement the service layer and the application layer. As mentioned earlier, to achieve platform independence, the implementation is all done in Java and JSP.

\subsection{Service Layer Implementation}
\label{sec:service_layer_implementation}  

In this section, we explain the structure of our service layer code and define the interfaces provided by each component. As described earlier in section \ref{sec:serviceLayer}, the service layer includes five types of components, namely, Certificate Authority, Relay, Rendezvous and STUN Servers and the peer. The corresponding Java code for the service layer, is structured in a way that reflects the separation of these entities. As shown in Figure \ref{fig:overall_package}, the overall view of the service layer code lays out four different packages: \begin{itemize}
\item {\bf servers}: Which includes the implementation of the four server components of the service layer, each in a separate package.
\item {\bf net}: Which implements a secure socket over both UDP and TCP. This package includes {\bf SecureSocket} and {\bf rudp} packages. rudp package implements reliable UDP. The SecureSocket package implements a secure socket over TCP and reliable UDP, while its sub package {\bf RelaySocket}, implements a relayed secure socket.  
\item {\bf security}: Which implements security utilities needed by the other components.
\item {\bf peer}: Which implements the services available to peers as part of the interface used by MyZone engine in the application layer.
\end{itemize} 

Figure \ref{fig:net_package}, \ref{fig:rendezvous_package} and \ref{fig:peer_package} describe net, RendezvousServer and peer packages in more detail using UML class diagrams. 
The net package includes the rudp and SecureSocket packages. The rudp package is implemented using two classes: The {\bf ReliableSocket} class implements a reliable datagram client socket using the standard datagram socket provided by Java. The {\bf ReliableServerSocket} class implements a reliable datagram server socket using the ReliableSocket class. 

The SecureSocket package is composed of {\bf TLSClientSocket}, {\bf TLSServerSocket}, and {\bf SecureSocket} classes and {\bf RelaySocket} package. The TLSClientSocket and TLSServerSocket implement client and server side {\it TLS like} secure sockets respectively. The main functionalities of these two classes is to perform the certificate and session key exchanges required as part of TLS handshake. 

Upon successful exchange of the session key, a SecureSocket class is instantiated by each of these classes. The SecureSocket class performs send and receive functionalities, while encrypting all transmitted data using the exchanged session key. The RelaySocket package implements the same functionalities as TLSClientSocket and TLSServerSocket but specifically for a relayed connection. As mentioned earlier, the relayed connection is an end to end secure connection and can not be decrypted by the relay server.

The RendezvousServer package includes the {\bf rendezvousServer} class that implements the functionalities of the rendezvous server. The {\bf db} class implements the database driver needed by the RendezvousServer class to communicate with the rendezvous server database. The other classes are used to store data for peer, relay server and friendship requests. 

Finally, the peer package implements all the functionalities available to peers using the {\bf peer} class. The peer class uses {\bf discoverNat} to discover the type of NAT that the peer is behind, and stores this information in the {\bf discoveryInfo} class. As for the RendezvousServer package, all the other classes are used to represent optional data. Tables \ref{table:interfaces_p1}, and \ref{table:interfaces_p2} define all the interfaces for each of the components. 

\begin{figure} \begin{center} \scalebox{.3}{\includegraphics{overall_package.png}} \end{center}
\caption{Overall view of all the composing packages of the service layer and their relationships. \label{fig:overall_package} }
\end{figure}

\begin{figure} \begin{center} \scalebox{.3}{\includegraphics{net_package.png}} \end{center}
\caption{Class diagram for the net package. \label{fig:net_package} }
\end{figure}

\begin{figure} \begin{center} \scalebox{.3}{\includegraphics{rendezvous_package.png}} \end{center}
\caption{Class diagram for the RendezvousServer package. \label{fig:rendezvous_package} }
\end{figure}

\begin{figure} \begin{center} \scalebox{.3}{\includegraphics{peer_package.png}} \end{center}
\caption{Class diagram for the peer package. \label{fig:peer_package} }
\end{figure}

\begin{sidewaystable}
\caption{Description of the interfaces for Rendezvous Server, and Relay Server components of the service layer.} \label{table:interfaces_p1}
\centering
\begin{tabular}{|p{3.5cm}|p{5cm}|p{13cm}|}
\hline
Component & Interface & Description \\
\hline Rendezvous Server & {\tt RendezvousServer(int port, String dbUsername, String dbPassword, String dbURL, String sessionKeyType, String asymAlgorithm, String sessionCipher Algorithm, int age, int refreshInterval)} & 

$-$ port: the port number that this rendezvous server listens on.

$-$ dbUsername: the username for the mysql\footnote{We use mysql dbms for rendezvous server database.} account.

$-$ dbPassword: the password of the corresponding username for the mysql account.

$-$ dbURL: the url to the mysql database.

$-$ sessionKeyType: the type of the symmetric encryption key used for session encryption

$-$ asymAlgorithm: the type of the algorithm used for asymmetric encryption.

$-$ sessionCipherAlgorithm: the type of the symmetric encryption algorithm used for session encryption.

$-$ age: the maximum period of time that a relay server is kept in the relay servers table without being refreshed.

$-$ refreshInterval: the refresh/update interval for relay servers. This value needs to be less than the value of age.
\\
\hline Relay Server & {\tt RelayServer(String rendezvousSrvAddr, int rendezvousSrvPort, int port, int maxConnections, int pingInterval)} &

$-$ rendezvousSrvAddr: the address of the rendezvous server which this relay would register with. 

$-$ rendezvousSrvPort: the remote port to connect on the rendezvous server.

$-$ port: the port that the relay server would be listening on. 

$-$ maxConnection: the maximum number of serving connections that this relay can handle.

$-$ pingInterval: at the end of this interval each serving socket needs to send a {\tt SERVER\_IS\_ALIVE} packet so that the relay server keeps it registered in its connection list.
\\
\hline
\end{tabular}
\end{sidewaystable}

\begin{sidewaystable}
\caption{Description of the interfaces for Certificate Authority Server, STUN Server, and Peer components of the service layer.} \label{table:interfaces_p2}
\centering
\begin{tabular}{|p{3.5cm}|p{6cm}|p{11cm}|}
\hline
Component & Interface & Description \\
\hline Certificate Authority Server & {\tt CAServer(int port, int backlog, InetAddress bindAddr, String caName, String priKeyPath, String keyAlgorithm)} &

$-$ port: the port number that the server listens on.

$-$ backlog: the number of waiting clients in the backlog queue.

$-$ bindAddr: the InetAddress of the network interface that the server is going to use.

$-$ caName: the name of the certificate authority. This is mainly used by the CA to read its private and public keys.

$-$ priKeyPath: the path to the directory where the private key of CA is stored at.

$-$ keyAlgorithm: the algorithm that is going to be used to issue certificates.
\\
\hline STUN Server & {\tt StunServer(int primaryPort, InetAddress primary, int secondaryPort, InetAddress secondary)} & 

$-$ primaryPort: The port number for the first network interface.

$-$ primary: the inet address of the first network interface.

$-$ secondaryPort: The port number for the second network interface.

$-$ secondary: the inet address of the second network interface.
\\
\hline Peer & {\tt peer(String username, int port, String myCertPath, String caCertPath, String myKeyPath, String passphrase, byte[] mirrors)} & 

$-$ username: The username of the user.

$-$ port: The port number that the peer accepts connections on. 

$-$ myCertPath: The path to the directory that holds the user certificate.

$-$ myKeyPath: The path to the directory that contains the key pair of the user.

$-$ passphrases: The list of passphrases for the user. Each passphrase corresponds to a single friendship

$-$ mirrors: The list of mirrors for the user. The list includes the usernames of all friends that have accepted to mirror the user profile on their machine.\\
\hline
\end{tabular}
\end{sidewaystable}

\subsection{Application Layer Implementation}
\label{sec:application_layer_impelentation}

\begin{figure} \begin{center} \includegraphics[width=\textwidth]{application_layer_class_diagram.png} \end{center}
\caption{Class diagram for the entire application layer. \label{fig:application_layer} }
\end{figure}

In this section we explain how our design architecture for the application layer, shown in Figure \ref{fig:design_architecture} is implemented. As we described in \ref{sec:applicationLayer}, the application layer has three major components, namely, the MyZone Engine, the web application and the shared classes. Figure \ref{fig:application_layer} shows all the classes that implement the application layer and their relationships with each other in form of a UML class diagram. 


The class diagram can be viewed as having three separate components corresponding to those in the application layer design. The main class in the MyZone Engine component shown at the top, is {\bf MyZoneEngine} which is composed of two subclasses: {\bf servingThread} and {\bf clientThread}. The two subclasses correspond to the two subcomponents of the MyZone Engine component. Note that during the entire lifetime of MyZone engine there exists only one instance of these classes. The clientThread class has three subclasses each implementing one of the three tasks that the clientThread class is responsible for, as described in \ref{sec:applicationLayer}. These three subclasses use the shared classes in order to operate on data stored in form of XML files. 

The servingThread has only one subclass called {\bf server}. For each request received at the serving socket instantiated in the servingThread class, an instance of server class is created to handle the request based on its type. The three functions, {\bf sync}, {\bf receiveUpdates}, and {\bf sendUpdates} are responsible for synchronization with an original device, posting updates and sending updates requests respectively. At the end of serving a request, the server class calls the {\bf cleaner} class which manages the storage by deleting the oldest files in case the maximum set capacity has reached. 


The web application component in Figure \ref{fig:design_architecture} is implemented using two packages: The Jetty web server and the JSP files. The Jetty web server is an open source web server completely written in Java and supports JSP files. Each JSP file in the JSP package implements a single web interface in form of a dynamic web page. The index.jsp file {\it represents the news feeds for different zones} and {\it the user can use this interface to like, dislike, or comment on any content shown on her news feed} (Figure \ref{fig:feed_ss}). The profile.jsp file {\it converts all the profile information of a user stored as XML files, to a web page}. The user can use the provided interface to {\it post contents on her own profile or a friend's profile} (Figure \ref{fig:profile_ss}). The messages.jsp file {\it converts all the private messages sent to the user from XML format to a web page}. It also {\it provides the required web interfaces for the user to compose private messages to her friends} (Figure \ref{fig:message_ss}). The events.jsp file is responsible for {\it representation, as well as modification and creation of events} (Figure \ref{fig:event_ss}). The friends.jsp file {\it shows the list of all friends} and enables the user to {\it delete a friend}, {\it send a request for friendship} and {\it accept or deny a received friendship request} (Figure \ref{fig:friend_ss}). The mirrors.jsp file (Figure \ref{fig:mirror_ss}) shows all the settings related to mirrors and provides the following functionalities to the user:
\begin{itemize}
\item Sending mirroring requests to other friends.
\item Accept or deny received mirroring requests.
\item Delete a user from the list of mirrors.
\item Change the rank of a mirror.
\item Refuse to mirror a particular friend. 
\item Change the allocated storage for mirroring a particular friend.
\end{itemize}
Finally, settings.jsp displays all the settings for the client application and provides the interface to modify all the setting attributes listed in Table \ref{table:settings_attributes} (Figure \ref{fig:settings_ss}). In addition it provides the interface to manage zones, enabling users to create, delete or modify the members of a zone (Figure \ref{fig:zone_ss}). Since all data is stored in XML files, all the JSP files use shared classes in order to operate on the XML files. The shared classes component acts as a toolkit for MyZone engine and web application components. The shared classes package includes a package called elements. This package has a corresponding class for every XML element used in MyZone and each class is primarily responsible for converting the XML elements to Java objects and vice versa.  

\begin{figure} \begin{center} \includegraphics[width=\textwidth]{feed_ss.png} \end{center}
\caption{A snapshot of the web interfaces implemented by index.jsp. \label{fig:feed_ss} }
\end{figure}

\begin{figure} \begin{center} \includegraphics[width=\textwidth]{profile_ss.png} \end{center}
\caption{A snapshot of the web interfaces implemented by profile.jsp. \label{fig:profile_ss} }
\end{figure}

\begin{figure} \begin{center} \includegraphics[width=\textwidth]{message_ss.png} \end{center}
\caption{A snapshot of the web interfaces implemented by messages.jsp. \label{fig:message_ss} }
\end{figure}

\begin{figure} \begin{center} \includegraphics[width=\textwidth]{event_ss.png} \end{center}
\caption{A snapshot of the web interfaces implemented by events.jsp. \label{fig:event_ss} }
\end{figure}

\begin{figure} \begin{center} \includegraphics[width=\textwidth]{friends_ss.png} \end{center}
\caption{A snapshot of the web interfaces implemented by friends.jsp. \label{fig:friend_ss} }
\end{figure}

\begin{figure} \begin{center} \includegraphics[width=\textwidth]{mirror_ss.png} \end{center}
\caption{A snapshot of the web interfaces implemented by mirrors.jsp. \label{fig:mirror_ss} }
\end{figure}

\begin{figure} \begin{center} \includegraphics[width=\textwidth]{settings_ss.png} \end{center}
\caption{A snapshot of the web interfaces implemented by settings.jsp. \label{fig:settings_ss} }
\end{figure}

\begin{figure} \begin{center} \includegraphics[width=\textwidth]{zone_ss.png} \end{center}
\caption{A snapshot of the web interfaces implemented by settings.jsp that manages the zones. \label{fig:zone_ss} }
\end{figure}

\begin{table}
\caption{MyZone setting attributes for the application layer.} \label{table:settings_attributes}
\centering
\begin{tabular}{|p{4cm}|p{11cm}|}
\hline
Setting Attribute & Description \\
\hline 

Number of entries per wall session & This number indicates the maximum number of profile contents represented as xml elements stored in one xml file as explained in section \ref{sec:applicationLayer} and needs to be between $100$ and $1000$. As this number grows, the number of XML files decreases while the individual file sizes increase making searching within a file slower. The default value for this attribute is $100$.\\
\hline
Rendezvous Server Address & The IP address of the rendezvous server that the client needs to register with.\\
\hline
Rendezvous Server Port & The port number for the rendezvous server that the client needs to register with.\\
\hline
STUN Server Address & The IP address of the STUN server.\\
\hline
STUN Server Port & The port number for the STUN server.\\
\hline
MyZone Server Port & The local port number that MyZone engine is listening on for requests from other peers.\\
\hline
MyZone Cache Size & The limit on the size of the friends directory where all friends' profiles are stored in.\\
\hline
Priority of this device & This attribute indicates whether the current device is primary, secondary or tertiary.\\
\hline
Synchronization period & This attribute indicates how often this device should synchronize with lower priority devices and other mirrors. A smaller period results in more frequent synchronizations which translates into more traffic while a larger period results in more inconsistent profile images on mirrors as synchronization is done less frequently.\\
\hline
\end{tabular}
\end{table}

After describing the code structure of the application layer in terms of its composing classes and their relationships, we proceed to explain how data is managed in the application layer. Data in MyZone can be categorized into three groups: 
\begin{itemize}
\item Client application settings.
\item User specific data.
\item Profile information.
\end{itemize}

With the exception of the client application settings, all data are stored under a directory named after the username of the device owner. The client application settings are described in Table \ref{table:settings_attributes} and stored in settings.xml. Table \ref{table:settings} in Appendix \ref{ch:appendix} describes the XML schema of settings.xml. 

The user specific data is composed of the following items:
\begin{itemize}
\item User mirroring information which includes the list of mirrors stored in {\bf mirrors.xml}, the list of mirrored users stored in {\bf originals.xml} and the lists of sent mirroring requests and received mirroring requests stored in {\bf sentMirroringRequests} and {\bf receivedMirroringRequests.xml} respectively. Table \ref{table:mirror} in Appendix \ref{ch:appendix} describes the XML schema of the mirror element. 
\item List of friends, received friendship requests and sent friendship requests stored in {\bf friends.xml}, {\bf awaitingFriendships.xml} and {\bf pendingFriendships.xml}. Table \ref{table:friends} describes the XML schema of the friend element. 
\item List of all passphrases. Each passphrase corresponds to a unique friendship. The list of passphrases is stored in {\bf passphrases.xml} and Table \ref{table:passphraseEntry} in Appendix \ref{ch:appendix} describes the XML schema of the passphrase entry element.  
\item List of all zones and their settings including members of each zone stored in {\bf zones.xml}. Table \ref{table:zone} in Appendix \ref{ch:appendix} describes the schema of the zone element.
\item List of all files that make up the correct file system image stored in {\bf correctImage.xml}. Each entry in this list includes the filename and its size as described in Table \ref{table:fileList} in Appendix \ref{ch:appendix}. There are two kinds of files that are included in correctImage.xml: The files that belong to friends' profiles which are considered as part of cache storage, and the files that belong to the device owner's profile or other mirrored profiles. 
\item List of all files that make up the existing file system image stored in {\bf existingImage.xml}. Each entry in this list is similar to those in correctImage.xml. The cleaner thread computes the correct image and manages the storage by deleting all the files for entries that are only in existingImage.xml and not in the correctImage.xml.
\end{itemize} 

The profile information can also be divided into three groups based on the ownership of profile, namely, the device owner, the mirrored users, and friends. The profile information is composed of the following items:
\begin{itemize}
\item Information about the user stored in {\bf info.xml}. This includes both basic information as well as employment and education history which are optional. Table \ref{table:info} in Appendix \ref{ch:appendix} describes the XML schema of the elements in info.xml. 
\item User events including both the events she has created and those that she is invited to which are stored in {\bf events.xml}. Table \ref{table:event} in Appendix \ref{ch:appendix} describes the XML schema of the event element
\item Sent and received private messages stored in {\bf outbox.xml} and {\bf inbox.xml} respectively. Table \ref{table:messages} in Appendix \ref{ch:appendix} describes the XML schema of a message element. The sent and received private messages are encrypted using the private key of the sender and the public key of the receiver and are safe to be stored on mirrored devices as they can not be decrypted by anyone except the intended receiver. 
\item Profile entries as posts. The entries can be status updates or message posts which we refer to as wall posts, as well as links, photos, audios, and videos. The user can organize photo, audio, and video posts as albums. Tables \ref{table:wallPost}, \ref{table:link}, \ref{table:photo}, \ref{table:audio} and \ref{table:video} in Appendix \ref{ch:appendix} describe the XML schemas for profile entries. Note that each element has three sub elements that correspond to likes, dislikes and comments posted on that profile entry. As each of these profile entries may be deleted by its owner at some point, we use an XML element called deletedEntry in order to keep track of deleted entries. Table \ref{table:deletedEntry} in Appendix \ref{ch:appendix} describes the XML schema of a deletedEntry element.
\item Finally, all the profile entries posted on another friend's profile are initially stored in {\bf pendingChanges.xml} and are removed upon successful submission by the postingThread of the clientThread. Table \ref{table:pendingChange} in Appendix \ref{ch:appendix} describes the XML schema of the pendingChange element. 
\end{itemize}

All of the above items are stored for the device owner's profile whereas for a mirrored profile the pending changes are not stored and for friends' profiles only the profile entries are stored locally. This concludes our overview of the implementation of MyZone which includes over seventeen thousands lines of code for the service layer and just under thirty thousands lines of code for the application layer excluding the Jetty web server. In the next chapter we evaluate the local deployment of MyZone with respect to availability, scalability and resource utilization.  



==> securityMeasures.tex <==
\section{Security Measures}
\label{ch:securityMeasures}

In section \ref{sec:serviceLayer} we described the design of the service layer without considering security attacks. In this section we explain the possible security attacks, the scenarios that implement them, and the measures taken to detect, prevent, and recover from these attacks. Furthermore, we modify the design of the service layer to incorporate these measures. We start by identifying all the security attacks that apply to our peer to peer OSN environment and defining the scenarios that implement them. Then, we describe a modified peer registration process for the global deployment model, that embodies our security measures. Finally we explain how the design handles the attacks. 

The adversary model was defined earlier in \ref{subsubsec:adversary} where we described the malicious entities, their resources and the types of attacks that they can implement. Here, we further categorize the adversaries into three groups:
\begin{enumerate}
\item Those that try to hijack user information i.e. profile, friend list, etc.
\item Those that try to isolate particular peers, or groups of peers from other users.
\item Those that try to make the system unresponsive by attacking its server components.
\end{enumerate}

As a reminder from earlier, we state that a malicious node can be any component of the system with the exception of the certificate authority. This essentially means that any rendezvous or relay server or peer can be malicious\footnote{As mentioned earlier in \ref{subsubsec:trustmodel}, a peer would not act maliciously towards its own friends}. Note that these assumptions only apply to the global deployment model, as opposed to the local deployment model where the goal of constructing a private OSN would require the components to be trustworthy. 

In addition, any malicious node can choose selectively to act correctly or maliciously towards other components. Based on these assumptions any attack that attempts to use impersonation e.g. man in the middle, spoofing, eavesdropping etc. will not be a concern since we assume that all components of the system with the exception of the certificate authority and friends are not trusted. However, the design uses a decentralized technique that detects and isolates the malicious entities over time, as will be explained later on. 


\subsection{Security Attacks and Scenarios}
\label{subsec:scenarios}

The security attacks that apply to our model and their corresponding scenarios are:
\begin{itemize}
\item {\bf Sybil attacks}: an attacker creates a large number of identities and dominates the overlay network by fooling the protocols, and subverting mechanisms based on redundancy.

Scenario:
\begin{itemize} 
\item {\bf S.1}) A malicious node creates virtual rendezvous servers and tries to take over a particular key (username) or pollute the routing tables of the other rendezvous servers.
\end{itemize}
\item {\bf Eclipse attacks} also known as routing table poisoning: an attacker controls a sufficient fraction of the neighbors of a node, hence the node can be ÒeclipsedÓ. This kind of attack applies to network proximity based DHTs like Pastry\cite{pastry} and Tapestry\cite{tapestry} and is very hard to achieve in Chord. 

Scenario:
\begin{itemize}
\item {\bf E.1}) A set of malicious rendezvous servers try to target (eclipse) a particular correct rendezvous server by poisoning the routing tables of other rendezvous servers.
\end{itemize}
\item {\bf Routing attacks}: an attacker may do a combination of the following:
\begin{itemize}
\item Refuse to forward a lookup request. 
\item It may forward it to an incorrect, non-existing, or malicious node. 
\item It may pretend to be the node responsible for the key.
\end{itemize}

Scenarios:
\begin{itemize}
\item {\bf R.1, R.2, R.3}) Malicious rendezvous servers do one or some combination of the above, on a locate rendezvous server request shown in Figure \ref{fig:dht_registration}.
\end{itemize}
\item {\bf Storage attacks}: a node routes requests correctly, but denies the existence of a valid key or provides invalid data as response. This attack can be in conjunction with the routing table attack.

Scenario:
\begin{itemize}
\item {\bf T.1}) A rendezvous server returns incorrect information in response to a locate peer request.
\end{itemize}
\end{itemize}
 
\subsection{Security Measures}
 \label{subsec:measures}
 
Now that we have defined the security attacks and their corresponding scenarios, we can introduce the modified peer registration process. This modification only applies to the global deployment model that uses chord DHT. Figure \ref{fig:modified_dht_registration} shows the overall registration process in the global deployment model. 


The process is modified to reflect the fact that although the peers initially assume that the rendezvous servers are acting correctly, they don't trust them until their behaviors are verified by another trusted entity. Rendezvous server $X$ corresponds to the initial rendezvous server $R_k$ in Figure \ref{fig:dht_registration}, while $Y$ and $Z$ correspond to the rendezvous servers {\it assumed to be} responsible for MD5 and SHA-1 hashed username values respectively. 

\begin{figure*} \begin{center} \includegraphics[width=\textwidth]{modified_dht_registration.pdf} \end{center}
\caption{The modified peer registration process for the global deployment model. \label{fig:modified_dht_registration} }
\end{figure*}

The modified process is executed before peer $i$ registers with the rendezvous servers. Using this process peer $i$ can  verify if $Y$ and $Z$ are really responsible for its keys, or if they are malicious nodes trying to take over $i$. The process is summarized in Algorithm \ref{alg:modifiedRegistration}.

\begin{algorithm}
\caption{Modified registration process.}
\label{alg:modifiedRegistration}
\begin{algorithmic}[1]
\STATE randomly choose a rendezvous server $X$.
\STATE $(Y, Z) = X.LocateRendezvousServers(MD5(i), SHA-1(i))$;
\FORALL{friends $j$ of $i$}
\STATE $(R, S) = Y.LocateRendezvousServers(MD5(j), SHA-1(j))$; \COMMENT{steps 1 and 2 in Figure \ref{fig:modified_dht_registration}.}
\STATE $(T, U) = Z.LocateRendezvousServers(MD5(j), SHA-1(j))$; \COMMENT{steps 1 and 2 in Figure \ref{fig:modified_dht_registration}.}
\STATE $(CI_j(R))=R.LocatePeer(j)$;  \COMMENT{steps 3 and 4 in Figure \ref{fig:modified_dht_registration}. $CI_j(R)$ denotes the connection information for peer $j$ obtained from rendezvous server $R$.}
\STATE $(CI_j(S))=S.LocatePeer(j)$; \COMMENT{steps 3 and 4 in Figure \ref{fig:modified_dht_registration}}
\STATE $(CI_j(T))=T.LocatePeer(j)$; \COMMENT{steps 3 and 4 in Figure \ref{fig:modified_dht_registration}}
\STATE $(CI_j(U))=U.LocatePeer(j)$; \COMMENT{steps 3 and 4 in Figure \ref{fig:modified_dht_registration}}
\IF[At least one of the connection information was correct and a connection has been successfully established to $j$.] {$i.ConnectTo(CI_j(R)) \neq false \|  i.ConnectTo(CI_j(S)) \neq false \| i.ConnectTo(CI_j(T)) \neq false \| i.ConnectTo(CI_j(U)) \neq false$}
\STATE $(A, B)=D.LocateRendezvousServers(MD5(i), SHA-1(i))$; \COMMENT{steps 5 and 6 in Figure \ref{fig:modified_dht_registration}. $D \in \{R, S, T, U\}$ where the correct $CI_j$ was obtained from.}
\IF {$A==Y$} 
\STATE $i$ registers with rendezvous server $Y$;
\ELSE
\STATE $i$ marks $Y$ and $X$ as potentially malicious nodes and goes to line $1$;
\ENDIF 
\IF {$B==Z$}
\STATE $i$ registers with rendezvous server $Z$;
\STATE return; \COMMENT{terminates.}
\ELSE 
\STATE $i$ marks $Z$ and $X$ as potentially malicious nodes and goes to line $1$;
\ENDIF
\ENDIF
\ENDFOR
\STATE goto line $1$;
\end{algorithmic}
\end{algorithm}

Algorithm \ref{alg:modifiedRegistration} is a randomized algorithm and can only be used after user $i$ is friend with at least one other user. Next, we analyze Algorithm \ref{alg:modifiedRegistration} and provide a formula that computes the expected number of runs for a successful registration. 

\subsubsection{Analysis of Algorithm \ref{alg:modifiedRegistration}}

Algorithm \ref{alg:modifiedRegistration} runs until three trusted rendezvous servers are found in which case it terminates at line $19$. There are three cases where the algorithm repeats itself. These cases correspond to lines $15$, $21$ and $25$. The first two cases i.e. lines $15$ and $21$ correspond to scenarios where rendezvous servers $X$ and either $Y$ or $Z$ (depending on whether line $15$ or $21$ is executed) are detected as malicious while line $25$ is executed only if none of $i$'s friends are online. Therefore, each unsuccessful execution of Algorithm \ref{alg:modifiedRegistration} by peer $i$ is either due to none of its friends being online or selecting a malicious rendezvous server at line $1$. 

As successive runs of Algorithm \ref{alg:modifiedRegistration} detect malicious rendezvous servers, they will be marked and removed from the pool of candidate rendezvous servers at line $1$. Therefore, this algorithm will eventually terminate assuming that at least one of $i$'s friends are online and there are at least three non malicious rendezvous servers. 

To analyze the algorithm mathematically, we introduce the following notations:
\begin{itemize}
\item $n$: Denotes $i$'s total number of friends.
\item $m$: Denotes the number of malicious rendezvous servers present.
\item $r$: Denotes the total number of rendezvous servers present.
\item $p_{on}$: Denotes the probability that a friend of $i$ is online. For simplicity, we are assuming that this probability is the same for all friends of $i$ which in general is not true.
\end{itemize}

A run of Algorithm \ref{alg:modifiedRegistration} is successful if at least one friend of $i$ is online and the three rendezvous servers $X$, $Y$ and $Z$ are non-malicious. Only a malicious rendezvous server returns other malicious rendezvous servers therefore the chances that all three or at least two of the rendezvous servers are malicious translates into the probability of $X$ being a malicious rendezvous servers. Based on this observation, the probability that the first run of Algorithm \ref{alg:modifiedRegistration} terminates in successful registration is computed as:

$P_1(Success) = p_{on}(1-\frac{m}{r})$

Consecutively, the probability that the first run of Algorithm \ref{alg:modifiedRegistration} is unsuccessful is:

$P_1(Failure) = 1 - P_1(Success) $

The probability of termination on the second run is the same as failure on the first run and success on the second run. This means that either none of $i$'s friends were online or that two malicious rendezvous servers were detected on the first run, in which case in the second run, they will be excluded from the selection process at line $1$. The probability of successful registration on the second run is therefore:

$P_2(Success) = P_1(Failure)p_{on}(1-\frac{m-2}{r})$

Respectively, the probability of failure on the second run is computed as:

$P_2(Failure) = 1 - P_2(Success) $

Based on the above, a generalized formula for the $n$'th successful run after $n-1$ failures is derived as follows:

$P_n(Success) = \prod_{i=1}^{n-1}P_i(Failure)(1-\frac{MAX(0, m-2(n-1))}{r})$ 

Finally the expected number of runs of Algorithm \ref{alg:modifiedRegistration} for a successful registration can be derived from the above probability distribution function which is based on the number of friends if $i$, as well as the total number of rendezvous servers and malicious rendezvous servers present on the DHT ring. Next, we explain how the overall design addresses different attack scenarios by prevention, detection, and recovery techniques. 

\subsubsection{Prevention}

Out of attack scenarios described in \ref{subsec:scenarios}, there are three scenarios that are prevented by our design:

\begin{itemize} 
\item A malicious node targets a particular peer to either render the user unreachable by DDoS attack or hijack information from the user. 

Solution: This requires the attacker having access to the user connection information. The connection information can be obtained in two ways: sending the correct passphrase of the user to the rendezvous server responsible for the target user, or through registering with a malicious rendezvous server. 

The passphrases are only shared with friends that are all trusted and will not act maliciously. Furthermore, targeting a specific peer by a malicious rendezvous server is very unlikely due to the key distribution properties of consistent hashing\cite{consistent_hashing}. 

Even if a malicious node somehow obtains the connection information of the peer, although a DDoS attack is feasible, unauthorized access to the user information is prevented. This is because, the connection is encrypted using symmetric encryption and the process used to exchange the session key uses keys from both parties. 

The key exchange process ensures that the session key is encrypted by the sending party, in a manner, that it can only be decrypted by the receiving party. This, guarantees authentication and integrity at the same time, preventing man in the middle and impersonation attacks. In addition, connections from non-friend peers are refused.

\item S.1) A malicious node creates virtual rendezvous servers and tries to take over a specific user or pollute the rendezvous server tables to target that user.

Solution: the consistent hashing guarantees the balanced distribution of the identifiers. Consequentially, although an attacker can create a lot of malicious virtual rendezvous servers, it can only take over a specific user $x$, if it can predict the IP address of $Successor(x)$. This requires the malicious user to be able to reverse the consistent hashing function which is known to be hard. 

\item E.1) A set of malicious rendezvous servers try to bypass (eclipse) a particular correct rendezvous server by poisoning the routing tables of other rendezvous servers.

Solution: Although this attack is not explicitly prevented, it is effective only in DHTs that are based on network proximity and does not apply to chord\cite{dht_sec_survey}. Furthermore, the two independent identifiers for each username i.e. MD5 and SHA-1, would very likely result in two independent paths to two different rendezvous servers. This makes eclipse attacks even less effective. 

\end{itemize}

\subsubsection{Detection}

Our design would be able to successfully detect the following attack scenarios as explained below:

\begin{itemize}
\item R.1) Malicious rendezvous server refuses to forward a locate rendezvous server request.

Solution: The peer tries to find another rendezvous server from a list of publicly available rendezvous servers until it receives a reply.
\item R.2, R.3) Initial malicious rendezvous server $X$ returns malicious nodes $Y$ and $Z$ in response to $LocateRendezvousServers(${\it MD5(i)}$, ${\it SHA-1(i)}$)$ sent by peer $i$ in the initial stage of registration.


Solution: Malicious behavior at the registration stage is detected using lines $15$ and $21$ of Algorithm \ref{alg:modifiedRegistration}.

\item T.1) A rendezvous server returns incorrect information in response to a locate peer request.

Solution: Incorrect registration information can be identified by comparing the hash value computed over $IP + Port + \dots$ with the signed hash value i.e. $E(Q_{peer})[IP + Port + \dots]$ introduced in section \ref{sec:serviceLayer}.

This mechanism can also be used by rendezvous servers to detect malicious rendezvous servers upon replication of data. This is done by each rendezvous server, verifying the authenticity and integrity of the registration information that it receives from other servers, before replicating it. If a rendezvous server receives a modified registration information, it will not forward or replicate it.

\end{itemize}

\subsubsection{Recovery}

The biggest part of recovery is to isolate the malicious rendezvous servers after detection. The malicious rendezvous servers are removed by a collaborative decision making that uses a reputation based scheme. There are two ways to detect a malicious node: At the time of peer registration as described earlier, and After registration. 

Peer $i$ can detect malicious behavior of rendezvous server $X$ responsible for $i$, by receiving notifications from its friends who received incorrect or out of date registration information  from $X$, in response to {\tt locatePeer($i$)} queries. Note that in this scenario, $X$ has behaved correctly during the initial registration process otherwise $i$ would not have registered with $X$ from the beginning. 

Peer $i$ would send a complaint to a correct rendezvous server found in lines $13$ and $18$ of Algorithm \ref{alg:modifiedRegistration}. The complaint is spread on the chord ring and is recorded by the nodes that have an entry for $X$ in their routing tables. 

Server $X$ would be removed from the chord ring, only if the ring receives enough distinct complaints specifically from peers that are registered with $X$. The distinct complaints are required in order to prevent malicious peers from sending out falsified complaints, hence, removing a correct rendezvous server. 

If the received complaints regarding $X$ are not enough, the servers on the chord ring would agree not to isolate $X$, as it will be considered more beneficial than harmful. The benefit is the result of selective malicious behavior of $X$ towards peers. Respectively, peer $i$ would send a complaint only if it receives enough number of notifications from its friends. If these notifications are few, peer $i$ concludes that the benefit of $X$ still outdoes its harm. 

The complaint sent by any peer need to be authenticated. This means that the entire complaint needs to be signed by the peer and it should include a timestamp to prevent duplicated complaints. 

The described scheme is designed to impose the following restrictions:

\begin{enumerate}
\item A malicious rendezvous server should not be able to complain about a correct rendezvous server and only a peer registered with the rendezvous server should be able to complain about it.
\item A malicious peer can only complain about its own rendezvous server and only once. Therefore, if $r$ is the minimum number of complaints that are needed to exclude a node from the ring, then $r$ of these malicious peers need to register with the same rendezvous server to remove a specific rendezvous server. 
\item A peer can falsely believe that her rendezvous servers are malicious, only if her friends intentionally send notifications to her. This would result in unreachability of the peer and would violate the assumption that a peer would not act as adversary to her own friends.
\end{enumerate}
